YourBench: Easy Custom Evaluation Sets for Everyone

Evaluating large language models (LLMs) effectively remains a critical bottleneck, as traditional static benchmarks suffer from saturation and contamination, while human evaluations are costly and slow. This hinders timely or domain-specific assessment, crucial for real-world applications. We introduce YourBench, a novel, open-source framework that addresses these limitations by enabling dynamic, automated generation of reliable, up-to-date, and domain-tailored benchmarks cheaply and without manual annotation, directly from user-provided documents. We demonstrate its efficacy by replicating 7 diverse MMLU subsets using minimal source text, achieving this for under 15 USD in total inference costs while perfectly preserving the relative model performance rankings (Spearman Rho = 1) observed on the original benchmark. To ensure that YourBench generates data grounded in provided input instead of relying on posterior parametric knowledge in models, we also introduce Tempora-0325, a novel dataset of over 7K diverse documents, published exclusively after March 2025. Our comprehensive analysis spans 26 SoTA models from 7 major families across varying scales (3-671B parameters) to validate the quality of generated evaluations through rigorous algorithmic checks (e.g., citation grounding) and human assessments. We release the YourBench library, the Tempora-0325 dataset, 150k+ question answer pairs based on Tempora and all evaluation and inference traces to facilitate reproducible research and empower the community to generate bespoke benchmarks on demand, fostering more relevant and trustworthy LLM evaluation.

==> content/sections/future_work.tex <==
\paragraph{Towards a General Theory of Generated Benchmarks.}
Although Eq.~\eqref{eq:d2eg} provides a concise mathematical framework, many open theoretical questions remain. For instance:
\begin{itemize}
    \item \textbf{Optimal versus Heuristic Coverage.} Quantifying how well greedy or ensemble search approximates global coverage remains uncharted territory, hinting at future investigations of approximation factors or specialized coverage theorems.
    \item \textbf{Diversity and Information Gain.} Formalizing diversity within question sets has strong connections to submodular optimization, but new metrics are needed to capture the multifaceted aspects of language-model evaluation.
    \item \textbf{Verifiability Constraints.} Ensuring each question is grounded in document content suggests a rich line of work in robust QA validation, bridging textual entailment frameworks with evaluation set generation.
\end{itemize}

We hope that introducing D2EG and \eqref{eq:d2eg} invites future research on automated benchmark generation. By unifying question minimality, coverage, diversity, and verifiability, this framework aspires to supply large-scale language models with fast-evolving and richly structured testbeds, bridging real-world document complexity and systematic evaluation.


==> content/sections/limitations.tex <==
\section*{Limitations}

==> stylefiles/nips/imports.tex <==
% add template
\usepackage[final]{stylefiles/nips/neurips2024}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{graphicx}       % for graphics
\usepackage{amsmath}        % for math
\usepackage{xspace}         % for hflogo
\usepackage[colorinlistoftodos]{todonotes}
% \usepackage{authblk}
\usepackage{minted}
\setminted{
    frame=lines,
    framesep=2mm,
    baselinestretch=1.2,
    fontsize=\footnotesize,
    breaklines=true,
    linenos=true,
    numbersep=5pt,
    autogobble=true,
    mathescape=true
}
\usepackage{wrapfig}

\setminted[markdown]{
    % bgcolor=lightgray,
    breaklines=true,
    breakanywhere=true,
    fontfamily=tt,
    tabsize=2,
    linenos=false
}

\bibliographystyle{plainnat}
